Advancing Humanoid Locomotion: Mastering Challenging Terrains with Denoising World Model Learning

Humanoid robots, with their human-like skeletal structure, are especially suited for tasks in human-centric environments. However, this structure is accompanied by additional challenges in locomotion controller design, especially in complex real-world environments. As a result, existing humanoid robots are limited to relatively simple terrains, either with model-based control or model-free reinforcement learning. In this work, we introduce Denoising World Model Learning (DWL), an end-to-end reinforcement learning framework for humanoid locomotion control, which demonstrates the world's first humanoid robot to master real-world challenging terrains such as snowy and inclined land in the wild, up and down stairs, and extremely uneven terrains. All scenarios run the same learned neural network with zero-shot sim-to-real transfer, indicating the superior robustness and generalization capability of the proposed method.

==> Analysis/ankle.tex <==
% % \begin{figure}[tp]
% %     \centering
% %     \includegraphics[width=1\linewidth]{images/ankle_control.pdf}
% %     \caption{Dynamic Adaptation of the Ankle Control Mechanism. This series captures the humanoid robot's ankle control system effectively compensating for an externally applied perturbation force, underscoring the robustness of the control strategy.}
% %     \label{fig:ankle_control}
% %     \vspace{-0.15in}
% % \end{figure}

% \subsubsection{Benefits and Importance of Ankle Control}
% Compared to previous RL-based locomotion control for humanoid robots \cite{radosavovic2023learning}, another distinctive aspect of our work lies in ankle control. Through our indoor experiments, it becomes evident that ankle control is crucial for enabling robots to navigate through complex and challenging terrains.

% As our robot's ankle has two degrees of freedom: pitch and roll. Effectively controlling these two degrees of freedom can further contribute to maintaining the robot's balance. As illustrated in Fig. \ref{fig:ankle_control}, without ankle control, standing on a slope is unattainable. However, our method enables the robot to stand steadily on a slope, even resisting external disturbances and forces on the incline. This result is intuitive, as without ankle control, the robot would need to take steps or other actions when nearing tilting to maintain balance, making it impossible to achieve prolonged standing on the slope.

% During the traversal of uneven terrain and ascending stairs, the significance of ankle control in augmenting the robot's terrain adaptability becomes apparent. In our experiments, we observed that without ankle control, the robot's feet undergo substantial deformation upon contact with uneven terrain, rendering them unable to recover. Additionally, there is a lack of appropriate ankle joint contact forces, further increasing the likelihood of the robot losing balance and falling during subsequent foot placements. In contrast, our ankle control method effortlessly navigates through these terrains, providing additional ankle joint adaptive contact forces and reinforcing the robot's adaptability to different terrains.

\subsubsection{Benefits and Importance of Ankle Control}
Our work distinguishes itself from previous RL-based locomotion controls for humanoid robots \cite{radosavovic2023learning} through its emphasis on ankle control. Our experiments clearly demonstrate the critical role of ankle control in enabling robots to traverse complex and challenging terrains. 
Also, ankle control becomes particularly pronounced when walking on irregular blocks and ascending stairs as in Fig. \ref{fig:ankle_control}. We noted that without ankle control, the robot's feet deformed significantly upon contacting uneven ground, failing to recover. This was coupled with inadequate ankle joint contact forces, raising the risk of imbalance and falls during foot placements. In stark contrast, our ankle control method navigates these terrains with ease, by adaptive contact forces at the ankle joints as shown in the torque plot in Fig. \ref{fig:ankle_control}, enable robot's adaptability to varied terrains.


% The robot's ankles possess two degrees of freedom: pitch and roll. Effective management of these degrees of freedom is key to maintaining balance. As depicted in Fig. \ref{fig:ankle_control}, the absence of ankle control renders standing on a slope unfeasible. Conversely, with our approach, the robot stands stably on sloped surfaces, effectively countering external disturbances. Intuitively, lacking ankle control necessitates the robot to take steps or other corrective measures to avoid tilting, making sustained slope standing unachievable.



==> Introductions/intro.tex <==
% The achievement of agile and adaptive locomotion across diverse terrains is pivotal for the application of humanoid robots. 
\section{Introduction}

% 性能 real-world challenge terrain first end-to-end
% pure RL;achievement
% challenge terrain
% contribution: clear and strong


% intro 思路： 分成四个部分ABCD
% A. humanoid important



% B. classical control ZMP; MPC
% leak the ability of challenge terrain locomotion; optimization is hard

% C. RL is good for this purpose
% Cassie; robot dog show potential
% but humanoid is more harder
% bike not on challenge terrain

% D. Our work
% Achievement
% Zero-shot sim-to-real
% End-to-end drl
% Complex terrain
% Robust：Push cart; carry heavy load
% propose DWL first humanoid robot that masters challenge terrain
% snow, stair pure end-to-end RL, in Fig2
% zero shot sim2real transfer, same policy without fine-tune
% why we can do it: DWL (world model) only TS learn action; single phase training process; SRL
% ankle; passive ankle or point foot; cassie one dim; first Parallel Double-Linkage Ankle Mechanism and why that is important; robust





% Modern environments are primarily designed for humans, if agent .

% Modern environments are primarily designed for humans, humanoid robots have a similar skeletal structure to humans. Compared with other forms of robots, they have the potential to assist humans in completing various tasks in this human-center world.

Modern environments are primarily designed for humans. Therefore, humanoid robots, with their human-like skeletal structure, are especially suited for tasks in human-centric environments, offering unique advantages over other types of robots. To complete diverse tasks in real world, their mobility is crucial, underlining the necessity of their capacity to walk on complex terrains.

% so a robot capable of maneuvering through complex terrains is crucial for real-world applications. 

Traditional mobile robotic platforms often face substantial limitations in such environments. In contrast, humanoid robots, emulating the human body's structure, have the inherent potential to traverse varied landscapes and perform tasks like humans. However, unlike bipedal \cite{reher2019dynamic} or quadruped robots \cite{rudin2022learning}, humanoid need ensuring robustness as a higher center of gravity, instability during the swing phase, increased inertia in their legs, additional weight from the torso and arms, and their larger overall size.



% Why RL


% A. humanoid important
Recent advancements in model-free reinforcement learning (RL) have shown promise for developing adaptive legged locomotion \cite{rudin2022learning}. RL simplifies controller design by automating significant portions of the process and enables robots to learn adaptive behaviors in a variety of situations, which are often beyond the reach of traditional methods\cite{li2023robust}. In RL, robots are trained in a simulated environment to optimize a reward function, with the resulting policy then applied to the real robot. Despite its potential, RL faces several challenges, including bridging the significant gap between simulation and real-world physics, crafting appropriate reward functions for human-like walking, and the limited generality of RL algorithms, which may fail on atypical terrains.

% B. classical control ZMP; MPC
% leak the ability of challenge terrain locomotion; optimization is hard
In this work, we introduce a groundbreaking approach, \textbf{Denoising World Model Learning (DWL)}, for controlling humanoid robots on complex terrains. Unlike previous reinforcement learning (RL) efforts with bipedal robots like Cassie, which have achieved stair navigation and hard terrain traversal \cite{siekmann2021blind, siekmann2021sim}, our focus on humanoid robots presents a significantly more challenging setup. DWL excels in automating state representation learning \cite{lesort2018state}, mastering end-to-end learning for both prediction and adaptation, facilitating a seamless zero-shot transition to real-world scenarios, and effectively bridging the sim-to-real gap.

% C. RL is good for this purpose
% Cassie; robot dog show potential
% but humanoid is more harder
% bike not on challenge terrain

% D. Our work
% Achievement
% propose DWL first humanoid robot that masters challenge terrain
% snow, stair pure end-to-end RL, in Fig2
% zero shot sim2real transfer, same policy without fine-tune
% why we can do it: DWL (world model) only TS learn action; single phase training process; SRL
% ankle; passive ankle or point foot; cassie one dim; first Parallel Double-Linkage Ankle Mechanism and why that is important; robust




\begin{figure}[tp]
    \centering
    \includegraphics[width=0.7\linewidth]{images/ankle.pdf}
    \caption{Illustration of the humanoid robot's overall structure and the intricately designed Parallel Double-Linkage Ankle Mechanism. This mechanism is notable for offering two degrees of freedom in each ankle, enabling enhanced mobility and stability.}
    \label{fig:ankle}
    \vspace{-0.15in}
\end{figure}

% \begin{figure*}[htp]
%     \centering
%     \includegraphics[width=1\linewidth]{images/mian_plot_tmp_no_logo.png}
%     \caption{Extensive Showcase of Locomotion Using the DWL Framework. Displayed is a sequence illustrating a humanoid robot skillfully executing various locomotion tasks with the DWL framework in challenging environments. These include navigating snowy landscapes (A, K), ascending and descending stairs (B, J), crossing irregular terrains (I), and handling additional loads and dynamic forces (C, D, E, F, G, H). The robot also demonstrates its capability on slopes (L), highlighting DWL's adaptability and robustness in complex locomotion scenarios.}
%     \label{fig:main_exp}
%     \vspace{-0.15in}
% \end{figure*}

Conventional approaches, often encompassing multi-stage training processes \cite{agarwal2023legged}, complex reward designs \cite{yang2020learning}, or behavior cloning \cite{merel2018neural}, typically falter amidst the dynamic and unpredictable real-world scenarios. In contrast, DWL instead integrates a world model within an encoder-decoder framework, employing a masking loss to effectively predict the state from observations. This design functions as an efficient information bottleneck \cite{tishby2000information, tishby2015deep}, drawing inspiration from Masked AutoEncoders \cite{he2022masked, feichtenhofer2022masked, germain2015made, zhang2022survey} and the Model-Based RL algorithm \cite{hafner2019learning, hafner2019dream, hafner2020mastering}. The outcome is a methodology that not only ensures meaningful but also sparse learned representations, significantly enhancing the model's real-world transferability and effectiveness.

Our algorithm deployed on \textbf{StarBot} represents a major advancement for the field. The robot adeptly negotiates varied topography including uneven blocks, slopes, and stairs. This demonstrates both the practicality and robustness of the DWL algorithm. Notably, our controller, with only simulator training, directly transfers to the physical Xing-S3-bot without any tuning. To our knowledge, this marks the first RL-trained humanoid agent capable of reliably traversing stairs and other difficult terrain in real-world settings. Also, we tackle the complexities involved in simulating complex joint mechanisms, particularly the \textbf{Parallel Double-Linkage Ankle Mechanism}. Unlike others \cite{siekmann2021blind, reher2019dynamic}, our approach allows the agent to control two degrees of freedom of the ankle, enabling the StarBot to become extremely robust.



In summary, the DWL framework represents a groundbreaking advancement in the field of humanoid robotics, providing a novel and effective solution to the enduring challenges associated with sim-to-real transfer and operational adaptability in real-world settings. The key contributions of this work are threefold:
\begin{enumerate}
    \item Achieving a pioneering milestone with the StarBot, a real-world humanoid robot, successfully walking on complex terrains.
    \item Developing and implementing the innovative DWL framework, which demonstrates robust performance and significantly narrows the sim-to-real gap.
    \item Introducing and employing the Parallel Double-Linkage Ankle control, an innovative control strategy that substantially enhances the stability and flexibility of humanoid robotic movement.
\end{enumerate}


